FLERT: Document-Level Features for Named Entity Recognition

Current state-of-the-art approaches for named entity recognition (NER) typically consider text at the sentence-level and thus do not model information that crosses sentence boundaries. However, the use of transformer-based models for NER offers natural options for capturing document-level features. In this paper, we perform a comparative evaluation of document-level features in the two standard NER architectures commonly considered in the literature, namely "fine-tuning" and "feature-based LSTM-CRF". We evaluate different hyperparameters for document-level features such as context window size and enforcing document-locality. We present experiments from which we derive recommendations for how to model document context and present new state-of-the-art scores on several CoNLL-03 benchmark datasets. Our approach is integrated into the Flair framework to facilitate reproduction of our experiments.

==> tables.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\hline
 Approach &  \textsc{En} & \textsc{De} & $\textsc{De}_{06}$ & \textsc{Nl} & \textsc{Es} \\ \hline
 \textsc{\textit{XLM-R}}   & & & & & \\ 
 - Fine-tuning & \textbf{93.89 $\pm$ 0.12} & 87.12 $\pm$ 0.08 & 91.55 $\pm$ 0.07 & 94.20 $\pm$ 0.25 & 90.14 $\pm$ 0.14 \\
 - Feature-based & 93.12 $\pm$ 0.14 & 84.86 $\pm$ 0.11 & 89.88 $\pm$ 0.26 & 91.73 $\pm$ 0.21 & 88.98 $\pm$ 0.11\\ 
 - Proposed & 93.65 $\pm$ 0.09 & 86.99 $\pm$ 0.25 & 91.42 $\pm$ 0.08 & & 89.92 $\pm$ 0.27 \\
 - Proposed + WE &  93.55 $\pm$ 0.07 & 86.85 $\pm$ 0.20 & 91.46 $\pm$ 0.16 & & 89.88 $\pm$ 0.35 \\   \hline
%  \textsc{\textit{RoBERTa}}   & &&& & \\ 
%  - Fine-tuning &  93.13 &  &  & & \\ 
%  - Feature-based &  93.54 &  &  & & \\ 
%  - Proposed & \textbf{93.8} &  &  & & \\   \hline
 \citet{akbik2019naacl} & 93.18 $\pm$ 0.09 & - & 88.27 $\pm$ 0.30 & 90.44 $\pm$ 0.20 & - \\
 \citet{yu-etal-2020-named} & 93.5 & 86.4 & 90.3 & 93.7 & 90.3 \\
 \citet{strakova-etal-2019-neural} & 93.38 & 85.10 & - & 92.69 & 88.81 \\ \hline
 
\end{tabular}%
}
\caption{Comparative evaluation of proposed approach against baselines.}
\label{tab:dataset_stats}
\end{table*}

\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\hline
 Approach &  \textsc{En} & \textsc{De} & $\textsc{De}_{06}$ & \textsc{Nl} & \textsc{Es} \\ \hline
 \textsc{\textit{XLM-R}}   & & & & & \\ 
 - Fine-tuning + Dev & 93.96 $\pm$ 0.11 & 88.21 $\pm$ 0.43 & 92.29 $\pm$ 0.18 & 94.66 $\pm$ 0.12 & 89.93 $\pm$ 0.03 \\
 \hline
%  \textsc{\textit{RoBERTa}}   & &&& & \\ 
%  - Fine-tuning &  93.13 &  &  & & \\ 
%  - Feature-based &  93.54 &  &  & & \\ 
%  - Proposed & \textbf{93.8} &  &  & & \\   \hline
 \citet{akbik2019naacl} & 93.18 $\pm$ 0.09 & - & 88.27 $\pm$ 0.30 & 90.44 $\pm$ 0.20 & - \\
 \citet{yu-etal-2020-named} & 93.5 & 86.4 & 90.3 & 93.7 & 90.3 \\
 \citet{strakova-etal-2019-neural} & 93.38 & 85.10 & - & 92.69 & 88.81 \\ \hline
 
\end{tabular}%
}
\caption{Final evaluation with training + development set of fine-tuning approach against baselines.}
\label{tab:dataset_stats}
\end{table*}

\begin{table*}[ht]
\centering
\begin{tabular}{lll}
\hline
 Approach & \textsc{De} & $\textsc{De}_{06}$ \\\hline
 German BERT (deepset) & 83.77 $\pm$ 0.06 & 88.38 $\pm$ 0.27 \\
 German BERT (DBMDZ) & 85.77 $\pm$ 0.13 & 89.56 $\pm$ 0.55 \\
 GELECTRA & 87.63 $\pm$ 0.21 & \\
 \hline
 \citet{akbik2019naacl} & - & 88.27 $\pm$ 0.30 \\
 \citet{yu-etal-2020-named} & 86.4 & 90.3 \\
 \citet{strakova-etal-2019-neural} & 85.10 & - \\ \hline
\end{tabular}%
\caption{Comparative evaluation of monolingual German BERT models against baselines.}
\label{tab:dataset_stats}
\end{table*}

\begin{table*}[ht]
\centering
\begin{tabular}{ll}
\hline
 Approach & \textsc{En} \\\hline
 \textit{Fine-tuning} & \\
  - RoBERTa (large) + Context & 93.84 $\pm$ 0.12 \\
  - RoBERTa (large) + Context + Dev & 93.97 $\pm$ 0.15\\
 \hline
 Fine-tuning + Feature-based (mean) & \\
  - RoBERTa (large) + Context & 93.82 $\pm$ 0.12 \\
  - RoBERTa (large) + Context + WE & 93.74 $\pm$ 0.20 \\
 \hline
 \citet{akbik2019naacl} & 93.18 $\pm$ 0.09 \\
 \citet{yu-etal-2020-named} & 93.5 \\
 \citet{strakova-etal-2019-neural} & 93.38 \\ \hline
\end{tabular}%
\caption{Comparative evaluation of monolingual English BERT models (Fine-Tuning + Context) against baselines.}
\label{tab:dataset_stats}
\end{table*}

\begin{table*}[ht]
\centering
\begin{tabular}{ll}
\hline
 Approach & \textsc{Es} \\\hline
 BETO & 89.16 $\pm$ 0.11 \\
 \hline
 \citet{akbik2019naacl} & - \\
 \citet{yu-etal-2020-named} & 90.3 \\
 \citet{strakova-etal-2019-neural} & 88.81 \\ \hline
\end{tabular}%
\caption{Comparative evaluation of monolingual Spanish BERT models (Fine-Tuning + Context) against baselines.}
\label{tab:dataset_stats}
\end{table*}

\begin{table*}[ht]
\centering
\begin{tabular}{ll}
\hline
 Approach & \textsc{Nl} \\\hline
 BERTje & 92.15 $\pm$ 0.12 \\
 mBERT & 91.30 $\pm$ 0.25 \\
 \hline
 \citet{akbik2019naacl} & 90.44 $\pm$ 0.20\\
 \citet{yu-etal-2020-named} & 93.7\\
 \citet{strakova-etal-2019-neural} & 92.69\\ \hline
\end{tabular}%
\caption{Comparative evaluation of monolingual Dutch BERT models (Fine-Tuning + Context) against baselines.}
\label{tab:dataset_stats}
\end{table*}



\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\hline
 Fine-tuning Approach &  \textsc{En} & \textsc{De} & $\textsc{De}_{06}$ & \textsc{Nl} & \textsc{Es} \\ \hline
 \textit{XLM-R}  & 92.79 $\pm$ 0.10 & 86.60 $\pm$ 0.43 & 90.04 $\pm$ 0.37 & 93.50 $\pm$ 0.15 & 89.94 $\pm$ 0.24 \\ 
 + WE & 92.90 $\pm$ 0.18 & 86.35 $\pm$ 0.19 & 90.32 $\pm$ 0.14 & 93.63 $\pm$ 0.26 & 89.49 $\pm$ 0.24\\ 
 + Context & 93.64 $\pm$ 0.05 & 86.99 $\pm$ 0.24 & \textbf{91.55 $\pm$ 0.07} & 93.99 $\pm$ 0.16 & \textbf{90.14 $\pm$ 0.14} \\ 
 + WE + Context & 93.72 $\pm$ 0.08 & \textbf{87.12 $\pm$ 0.08} & 91.47 $\pm$ 0.16 & 93.96 $\pm$ 0.15  & 89.85 $\pm$ 0.08\\  \hline
 \textit{XLM-R-CRF} & 92.88 $\pm$ 0.14 & 85.71 $\pm$ 0.16 & 90.07 $\pm$ 0.35 & 93.54 $\pm$ 0.14 & 89.66 $\pm$ 0.19\\   
 + WE &  92.80 $\pm$ 0.23 & 85.80 $\pm$ 0.28 & 89.94 $\pm$ 0.05 & 93.29 $\pm$ 0.46 & 89.66 $\pm$ 0.18\\ 
 + Context & \textbf{93.89 $\pm$ 0.12} & 86.88 $\pm$ 0.33 & 91.18 $\pm$ 0.14 & \textbf{94.20 $\pm$ 0.25} & 89.57 $\pm$ 0.02 \\ 
 + WE + Context & 93.65 $\pm$ 0.10 & 86.86 $\pm$ 0.17 & 91.09 $\pm$ 0.34 & 93.96 $\pm$ 0.08 & 89.96 $\pm$ 0.10\\\hline
%  \textsc{\textit{RoBERTa}}   & 92.82 & & & \\ 
%  + WE & 92.77 &  &  & \\ 
%  + Context & 93.91 &  &  & \\ 
%  + WE + Context &  93.76 &  &  & \\  \hline
%  \textit{RoBERTa-CRF} & 92.80 &  &  & \\   
%  + WE &   &  &  & \\ 
%  + Context & 93.76  &  &  & \\ 
%  + WE + Context &  &  &  & \\ \hline \hline
\end{tabular}%
}
\caption{Evaluation of fine-tuning approach.}
\label{tab:dataset_stats}
\end{table*}

\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\hline
 Feature-based Approach &  \textsc{En} & \textsc{De} & $\textsc{De}_{06}$ & \textsc{Nl} & \textsc{Es} \\ \hline
 \textsc{XLM-R} (last 4 layers) &               &               &              &   83.12 $\pm$ 0.63          &   \\
 + WE &               &               &               &           84.39 $\pm$ 1.53       &   \\
 + Context &               &               &           &              85.67 $\pm$ 0.88    &   \\
 + WE + Context &               &               &               &      87.22 $\pm$ 0.17         &   \\  \hline
 \textsc{XLM-R} (all layer mean) &               &               &               &    89.47 $\pm$ 0.21         &   \\
 + WE &               &               &               &        90.91 $\pm$ 0.28         &   \\
 + Context &               &               &               &      91.63 $\pm$ 0.36        &   \\
 + WE + Context &               &               &               &     \textbf{92.52 $\pm$ 0.05}           &   \\   \hline
\end{tabular}%
}
\caption{Evaluation of feature-based approach (development set).}
\label{tab:dataset_stats}
\end{table*}


\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\hline
 Feature-based Approach &  \textsc{En} & \textsc{De} & $\textsc{De}_{06}$ & \textsc{Nl} & \textsc{Es} \\ \hline
%  \textsc{RoBERTa} (last 4 layers) &  &  &  & \\ 
%  + WE &  &  &  & \\ 
%  + Context &  &  &  & \\ 
%  + WE + Context &  &  &  & \\  \hline
%  \textsc{RoBERTa} (all layer mean) &  &  &  & \\ 
%  + WE &  &  &  & \\ 
%  + Context &  &  &  & \\ 
%  + WE + Context &  &  &  & \\\hline
 \textsc{XLM-R} (last 4 layers) & 87.85 $\pm$ 0.20 & 75.88 $\pm$ 1.73 & 80.66 $\pm$ 0.13 & 83.15 $\pm$ 1.17 & 86.09 $\pm$ 0.02 \\
 + WE & 88.91 $\pm$ 0.25 & 78.34 $\pm$ 0.60 & 81.13 $\pm$ 0.86 & 84.17 $\pm$ 1.93 & 86.28 $\pm$ 0.34 \\ 
 + Context & 91.47 $\pm$ 0.27  & 80.97 $\pm$ 1.09 & 84.61 $\pm$ 0.40 & 85.73 $\pm$ 1.00 & 86.46 $\pm$ 0.31 \\ 
 + WE + Context & 91.97 $\pm$ 0.19  & 81.85 $\pm$ 0.23 & 85.01 $\pm$ 0.46 & 87.75 $\pm$ 0.38 & 86.83 $\pm$ 0.41\\   \hline
 \textsc{XLM-R} (all layer mean) & 90.71 $\pm$ 0.04 & 81.53 $\pm$ 0.34 & 86.23 $\pm$ 0.29 & 89.24 $\pm$ 0.16 & 88.05 $\pm$ 0.36\\
 + WE & 91.83 $\pm$ 0.06 & 82.88 $\pm$ 0.28 & 87.35 $\pm$ 0.17 & 89.87 $\pm$ 0.45 & 88.78 $\pm$ 0.08\\ 
 + Context & 92.79 $\pm$ 0.11 & 84.68 $\pm$ 0.13 & 89.59 $\pm$ 0.33 & 91.58 $\pm$ 0.47 & 88.85 $\pm$ 0.11\\ 
 + WE + Context & \textbf{93.12 $\pm$ 0.14} & \textbf{84.86 $\pm$ 0.11} & \textbf{89.88 $\pm$ 0.26} & \textbf{91.73 $\pm$ 0.21} & \textbf{88.98 $\pm$ 0.11}\\   \hline
\end{tabular}%
}
\caption{Evaluation of feature-based approach. *only one run.}
\label{tab:dataset_stats}
\end{table*}
